A User-centered Security Evaluation of Copilot

Code generation tools driven by artificial intelligence have recently become more popular due to advancements in deep learning and natural language processing that have increased their capabilities. The proliferation of these tools may be a double-edged sword because while they can increase developer productivity by making it easier to write code, research has shown that they can also generate insecure code. In this paper, we perform a user-centered evaluation GitHub's Copilot to better understand its strengths and weaknesses with respect to code security. We conduct a user study where participants solve programming problems (with and without Copilot assistance) that have potentially vulnerable solutions. The main goal of the user study is to determine how the use of Copilot affects participants' security performance. In our set of participants (n=25), we find that access to Copilot accompanies a more secure solution when tackling harder problems. For the easier problem, we observe no effect of Copilot access on the security of solutions. We also observe no disproportionate impact of Copilot use on particular kinds of vulnerabilities. Our results indicate that there are potential security benefits to using Copilot, but more research is warranted on the effects of the use of code generation tools on technically complex problems with security requirements.

==> future.tex <==
% \section{Future Work}\label{sec:future_work}

% In order to verify whether Copilot does in fact make a significant difference on harder problems as suggested by the result (in our sample only) from RQ1, a more targeted user study may be required. Such a study would require a set of multiple problems, each with varying levels of difficulty. Ideally, we would want to establish a proxy for problem difficulty that can be compared to a proxy for security (like the security score in this user study) during analysis. The proxy for problem difficulty could be obtained from a number of sources including the time taken to solve problems or some aggregate of rankings of problem difficulty by users after they have solved the problems. Participants in the study would then be split into control and treatment groups, wherein the former solve all problems without Copilot and the latter solve all the problems with Copilot. We would then be able to measure how differences in security performance between the control and treatment group are affected by problem difficulty.

% The idea that the security impacts of Copilot could be more significant at higher levels of difficulty has implications for future research on and testing of Copilot and similar \glspl{cgt}. Mainly, it implies that testing \glspl{cgt} on trivial problems could yield misleading results. Researchers and developers of \glspl{cgt} may want to take steps to ensure that the problems upon which their tools are tested and evaluated are above a certain level of complexity, especially when the tools are being tested in conjunction with human users. For regular users of Copilot, a takeaway from the observations from our sample is the suggestion that Copilot can be especially helpful in writing more secure code when tackling more complex problems.
